MMP: Towards Robust Multi-Modal Learning with Masked Modality Projection

Multimodal learning seeks to combine data from multiple input sources to enhance the performance of different downstream tasks. In real-world scenarios, performance can degrade substantially if some input modalities are missing. Existing methods that can handle missing modalities involve custom training or adaptation steps for each input modality combination. These approaches are either tied to specific modalities or become computationally expensive as the number of input modalities increases. In this paper, we propose Masked Modality Projection (MMP), a method designed to train a single model that is robust to any missing modality scenario. We achieve this by randomly masking a subset of modalities during training and learning to project available input modalities to estimate the tokens for the masked modalities. This approach enables the model to effectively learn to leverage the information from the available modalities to compensate for the missing ones, enhancing missing modality robustness. We conduct a series of experiments with various baseline models and datasets to assess the effectiveness of this strategy. Experiments demonstrate that our approach improves robustness to different missing modality scenarios, outperforming existing methods designed for missing modalities or specific modality combinations.

==> acknowledgement.tex <==
\textbf{Acknowledgment:}
This work is supported in part by AFOSR award FA9550-21-1-0330 and an Amazon Gift award. This work used Indiana Jetstream2 through allocation CIS220128 from the ACCESS program supported by NSF grants 2138259, 2138286, 2138307, 2137603, and 2138296.
